Consistent but Miscalibrated: Evaluating LLM Limitations for Risk Communication in Natural Language

LLMs are increasingly deployed as post-hoc explainers of AI-generated outputs, yet it remains unclear whether they can reliably communicate probabilistic information in natural language. For this role to be viable, models must produce identical verbal descriptions for identical inputs, and select descriptions that accurately reflect the magnitude of the underlying numerical quantities. We evaluate whether nine LLMs meet these requirements within a two-stage prediction pipeline, in which an upstream model has produced probabilistic outputs characterized by their likelihood and uncertainty, and LLMs are tasked with selecting an appropriate verbal descriptor for each. We simulate predictions from an upstream model by taking samples from a Beta distribution parameterized by its mode and prior sample size. We then prompt LLMs to explain these predictions under six domain contexts and with ten temperature settings, and repeating each experiment ten times. We find that LLMs are generally consistent but miscalibrated, with substantially weaker performance on uncertainty than on likelihood tasks. Providing models with precomputed summary statistics (mode and prior sample size) reduced sensitivity to contextual framing but did not resolve the underlying miscalibration, suggesting that the bottleneck resides in the verbalization step itself. These findings indicate that current LLMs do not yet constitute reliable zero-shot standalone risk communication tools for probabilistic predictions.

==> sections/0-authors.tex <==

\author{Diego Cerda-Mardini \\
McGill University \\
Chandar Research Lab \\
Mila -- Quebec AI Institute \\
\texttt{diego.cerdamardini@mail.mcgill.ca} \\
\And
Sarath Chandar \\
Chandar Research Lab \\
Polytechnique Montr\'eal \\
Mila -- Quebec AI Institute \\
\And
Sreenath Madathil \\
McGill University \\
Mila -- Quebec AI Institute
}


==> sections/original_1-introduction.tex <==

\section{Introduction}

Large language models (LLMs) have demonstrated strong performance across a variety of natural language processing tasks and are increasingly deployed as the backbone of conversational agents \citep{brown2020language, openai2023gpt4}. Beyond text generation, recent research has extended LLMs into interactive and agentic settings, enabling tool use, planning, and long-horizon reasoning \citep{yao2023react, wang2024executable, rozanov2024stateact}. These systems typically operate under a standard chat interface, where the model conditions only on the public dialogue history to produce its next response. While this paradigm has proven effective for tasks that can be solved with context-limited reasoning or external retrieval \citep{lewis2020retrieval, borgeaud2022improving}, it implicitly assumes that all relevant state can be represented in the shared conversation, and that the agent has no need for private information inaccessible to the user. However, as LLMs are increasingly used as interactive agents, many tasks require them to maintain information privately across turns, something the standard chat paradigm does not support. This reveals a critical gap in the current literature.

Despite progress in memory and reasoning for LLM-based agents, current systems lack mechanisms for maintaining private working memory. While reasoning models can generate hidden intermediate states, standard chat interfaces do not persist them: internal reasoning tokens are discarded between turns \citep{openai_reasoning, openai_cookbook_gptoss_cot_2025, hf_transformers_chat_templating}. As a result, any privately generated state is immediately lost. Consider, for instance, the game of Hangman, in which a host privately selects a secret word and must reveal the positions of correct letters as a player makes guesses. When playing Hangman as the host, a model may internally select a secret word, but this choice is forgotten by the next turn, forcing the agent to hallucinate a new state. We document this behavior across major commercial interfaces in Appendix \ref{app:commercial_demo}.

Existing agentic frameworks such as ReAct and StateAct improve planning through structured reasoning and actions \citep{yao2023react, rozanov2024stateact}, but they are not designed to maintain hidden state across interactions. External memory systems, including RAG, Generative Agents, and related retrieval-based approaches, support long-term knowledge storage \citep{lewis2020retrieval, park2023generative, NEURIPS2023_1b44b878, wang2025rag+}, yet they do not capture dynamically generated, task-specific private state. Similarly, memory-focused systems such as LOCOMO \citep{maharana2024evaluating}, Mem0 \citep{chhikara2025mem0}, Memory-R1 \citep{yan2025memoryr1enhancinglargelanguage}, A-mem \citep{xu2025mem}, LightMem \citep{fang2025lightmem}, and MemoryOS \citep{kang2025memory} target public consistency, historical retrieval, or knowledge organization rather than secrecy or private state persistence. Cognitive architectures emphasize working memory and reasoning \citep{hu2024hiagent, sumers2023cognitive, li2025memos, hu2025unified}, but none enable agents to generate and preserve hidden information. Consequently, tasks that depend on private state, such as Hangman, remain unsolved. 

To formalize this gap, we introduce Private State Interactive Tasks (PSITs): interactive problems in which an agent must generate, preserve, and act consistently with hidden internal state while engaging in a dialogue. In PSITs, private beliefs must remain stable and aligned with public outputs without being revealed. Hangman is a canonical example: the agent must commit to a secret word and respond consistently to guesses. These tasks expose a structural limitation of standard chat-based agents, which cannot separate private state from public interaction. Without private working memory, agents fail to support a broad class of interactions, including games, role-play, negotiation, and tutoring, that fundamentally rely on hidden state.

\paragraph{Contributions.} 
We make three contributions. First, we formalize Private State Interactive Tasks (PSITs) and prove that standard chat-based LLMs are structurally incapable of solving them, since all information in the context is public by construction. This result identifies PSITs, exemplified by Hangman, as a distinct class of tasks beyond current LLM interfaces. Second, we propose and evaluate agent architectures that address this limitation by introducing a private working memory. We study three families: (i) Private Chain-of-Thought agents that preserve hidden reasoning across turns; (ii) Autonomous agents that independently decide when to invoke memory tools based on context; and (iii) Workflow-based agents that manage memory through a sequence of deterministic steps rather than dynamic decision-making. Each is tested under multiple memory update strategies. Third, we introduce a self-consistency testing protocol that evaluates whether an agent’s private memory remains aligned with its public behavior. Following an interaction where secrecy is strictly maintained, we fork the dialogue into a diagnostic probe where the agent is explicitly prompted to reveal its secret. This measures hidden–public coherence by checking if the agent consistently affirms its secret while rejecting alternatives, demonstrating the necessity of private working memory for reliable agents.

